Big Data Refinement

"Big data" has become a major area of research and associated funding, as well as a focus of utopian thinking. In the still growing research community, one of the favourite optimistic analogies for data processing is that of the oil refinery, extracting the essence out of the raw data. Pessimists look for their imagery to the other end of the petrol cycle, and talk about the "data exhausts" of our society. Obviously, the refinement community knows how to do "refining". This paper explores the extent to which notions of refinement and data in the formal methods community relate to the core concepts in "big data". In particular, can the data refinement paradigm can be used to explain aspects of big data processing?

==> eptcsdata.tex <==
\providecommand{\firstpage}{17}
\providecommand{\publicationstatus}{Eerke Boiten, John Derrick \& Steve Reeves (Eds.):\\
Refinement Workshop 2015 (Refine '15)\\
EPTCS 209, 2016, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.209.2}{10.4204/EPTCS.209.2}}

